On the Complexity of Computing Sparse Equilibria and Lower Bounds for No-Regret Learning in Games

Characterizing the performance of no-regret dynamics in multi-player games is a foundational problem at the interface of online learning and game theory. Recent results have revealed that when all players adopt specific learning algorithms, it is possible to improve exponentially over what is predicted by the overly pessimistic no-regret framework in the traditional adversarial regime, thereby leading to faster convergence to the set of coarse correlated equilibria (CCE). Yet, despite considerable recent progress, the fundamental complexity barriers for learning in normal- and extensive-form games are poorly understood. In this paper, we make a step towards closing this gap by first showing that -- barring major complexity breakthroughs -- any polynomial-time learning algorithms in extensive-form games need at least $2^{\log^{1/2 - o(1)} |\mathcal{T}|}$ iterations for the average regret to reach below even an absolute constant, where $|\mathcal{T}|$ is the number of nodes in the game. This establishes a superpolynomial separation between no-regret learning in normal- and extensive-form games, as in the former class a logarithmic number of iterations suffices to achieve constant average regret. Furthermore, our results imply that algorithms such as multiplicative weights update, as well as its \emph{optimistic} counterpart, require at least $2^{(\log \log m)^{1/2 - o(1)}}$ iterations to attain an $O(1)$-CCE in $m$-action normal-form games. These are the first non-trivial -- and dimension-dependent -- lower bounds in that setting for the most well-studied algorithms in the literature. From a technical standpoint, we follow a beautiful connection recently made by Foster, Golowich, and Kakade (ICML '23) between sparse CCE and Nash equilibria in the context of Markov games. Consequently, our lower bounds rule out polynomial-time algorithms well beyond the traditional online learning framework.

==> text/old-EFG.tex <==
\section{Sparse Coarse Correlated Equilibria}

We focus on the problem of computing \emph{sparse}---in the formal sense of \Cref{def:sparseCCE} below---coarse correlated equilibria (CCE) in multi-player games. More precisely, let us first recall the concept of a CCE in normal-form games, along with a certain refinement imposing a particular sparsity constraint.

\begin{definition}
[Sparse CCE]
    \label{def:sparseCCE}
    Let $\calG$ be an $n$-player game in normal form. A distribution over joint action profiles $\vec{\mu} \in \Delta\left( \prod_{i=1}^n \calA_i \right)$ is said to be an \emph{$\eps$-coarse correlated equilibrium ($\epsilon$-CCE)} if for any player $i \in [n]$ and deviation $a_i' \in \calA_i$,
    \begin{equation}
        \E_{\vec{a} \sim \vec{\mu}}[u_i(\vec{a})] \geq \E_{\vec{a} \sim \vec{\mu}}[u_i(a_i', \vec{a}_{-i})] - \eps.
    \end{equation}
    In particular, if $\vec{\mu}$ can be expressed as a uniform mixture of $k$ product distributions, $\vec{\mu}$ will be referred to as a \textit{$k$-sparse $\eps$-CCE}.
\end{definition}

Computing an $\eps$-CCE can be achieved in time $\poly(n, m, \log(1/\eps))$, where $m \triangleq \max_{1 \leq i \leq n} |\calA_i|$, for any game of polynomial type satisfying the polynomial expectation property~\citep{Papadimitriou08:Computing}. Here we are interested in the complexity of computing an approximate CCE under sparsity constraints, in the sense of~\Cref{def:sparseCCE}. A $1$-sparse CCE is clearly equivalent to a Nash equilibrium, thereby making the computational problem of finding a 1-sparse CCE $\PPAD$-hard~\citep{Daskalakis09:The}. On the other end of the spectrum, when $k = \poly(n, m, \log(1/\eps))$, there is a polynomial-time algorithm for finding a $k$-sparse CCE based on the Ellipsoid algorithm~\citep{Papadimitriou08:Computing}. Furthermore, specific no-regret learning algorithms, such as multiplicative weights update, yield an $O(\log m/\eps^2)$-sparse $\eps$-CCE in time $\poly(n, m, 1/\eps)$, again under the polynomial expectation property~\citep{Papadimitriou08:Computing}; we will be making the normalization assumption $|u_i(\vec{a})| \leq 1$ throughout. As a result, the key question that arises is to characterize the threshold of computational tractability in terms of the sparsity parameter $k$.

\section{Hardness of Sparse CCE in Extensive-Form Games}

We first focus on the problem of computing sparse CCE in extensive-form games. In particular, we assume that the game-tree is explicitly given as part of the input; we may also assume that every payoff at the leaves can be represented with a number of bits polynomial in the size of the game-tree. Extensive-form games are not of polynomial type given that a player's number of actions can be exponential in the description of the game. Nevertheless, polynomial (in the size of the game-tree) algorithms for computing (exact) CCE are known to exist; for example, \citet{Huang08:Computing} have shown how to adapt the Ellipsoid algorithm of~\citet{Papadimitriou08:Computing} for certain correlated equilibrium concepts in extensive-form games. (CCE per \Cref{def:sparseCCE} is typically referred to as \emph{normal-form} CCE (NFCCE) to differentiate with other notions of coarse correlation in extensive-form games.) Here we are interested in the complexity of the more refined concept introduced in~\Cref{def:sparseCCE}.

To prove hardness results for computing sparse CCE in extensive-form games, we rely on the reduction of~\citet{foster2023hardness}. In particular, we assume that we are given as input a two-player general-sum game where each player has $m \in \N$ actions; that is, $|\calA_1| = |\calA_2| = m$. We may also posit that every entry in the payoff matrices, say $\mat{M}_1, \mat{M}_2 \in \Q^{m \times m}$, can be represented with a number of bits polynomial in $m$. Moreover, we assume without any loss of generality that $|\mat{M}_1[a_1, a_2]|, |\mat{M}_2[a_1, a_2]| \leq 1$, for any combination of actions $(a_1, a_2) \in \calA_1 \times \calA_2$. Similarly to~\cite{foster2023hardness}, the key idea of the reduction is to show that a sparse CCE in a suitably constructed extensive-form game $\calG'$ (see \Cref{def:lifted-EFG}) can be used to obtain a Nash equilibrium in the original game $\calG$; in turn, the computational hardness of Nash equilibria in two-player game will preclude polynomial-time computation of sparse CCE under a certain sparsity regime (see \Cref{theorem:inference-EFGs}).

\begin{definition}[The lifted extensive-form game]
    \label{def:lifted-EFG}
We will consider extensive-form games with simultaneous moves; this comes without any essential loss since simultaneous moves can always be cast as sequential moves using imperfect information. So, the results we describe in the sequel apply to imperfect-information extensive-form games with sequential moves. 

Let $\calG$ be the original two-player game in normal form. The basic idea is to construct an extensive-form game $\calG'$ consisting of $H$ repetitions of $\calG$, for a sufficiently large parameter $H \in \N$ to be chosen later. More precisely, in each repetition $h \in [H]$, every player $i \in [2]$ selects an action $a_{i, h} \in \calA_i$ simultaneously with the other player. We will denote by $\calS$ the set of all possible states in the game, the set of all possible decision points (or information sets---trivially singleton in the present construction for both players) encountered in the game-tree. Finally, under a sequence of actions $(a_{i, 1}, \dots, a_{i, H}) \in \calA_i^H$ for each player $i \in [n]$, we assume that the utility of player $i \in [2]$ in the leaf-node corresponding to that combination of actions is given by $\frac{1}{H} \sum_{h=1}^H u_i(a_{1, h}, a_{2, h})$, where $u_i(\cdot)$ represents the utility function of player $i$ in the original game $\calG$; normalizing by the factor $H$ is to simply ensure that the payoffs in this induced extensive-form game are indeed in $[-1, 1]$.
\end{definition}

Based on this construction, the main reduction is summarized in \Cref{algo:EFG}. For the extensive-form game $\calG'$, we use $\vec{X}_i$ to represent the strategy of player $i$ in sequence form; the strategy induced by $\vec{X}_i$ at state $s \in \calS$ will be denoted by $\vec{X}_{i, s}$.

\begin{algorithm}[!ht]
    \caption{Reduction for \Cref{theorem:inference-EFGs}}
    \label{algo:EFG}
    \textbf{Input}: Two-player $m$-action game $\calG$ in normal form; accuracy $\epsilon > 0$; sparsity $T \in \N$ \\
    \textbf{Output}: A $(2\epsilon)$-Nash equilibrium of $\calG$\\
    Construct the two-player extensive-form game $\calG'(\calG)$ with $H \geq \frac{4 \log T}{\epsilon^2}$ (\Cref{def:lifted-EFG}) \\
    Compute a $T$-sparse $\epsilon$-CCE $\frac{1}{T} \sum_{t=1}^T \vec{X}_1^{(t)} \otimes \vec{X}_2^{(t)}$ \\
    \For{$s \in \calS(\calG'), t \in [T]$}{
    \If{$(\vec{X}_{1, s}^{(t)}, \vec{X}_{2, s}^{(t)}) \in \Delta(\calA_1) \times \Delta(\calA_2)$ is a $(2\epsilon)$-Nash equilibrium of $\calG$}{\textbf{return} $(\vec{X}_{1, s}^{(t)}, \vec{X}_{2, s}^{(t)})$} \label{line:return}
    }
    \textbf{return} \textsf{FAIL}
\end{algorithm}


Now the first important observation regarding $\calG'$ is that the number of nodes in the induced game-tree---incidentally coinciding with the cardinality of $\calS$ due to the structure of the game---can be expressed as $1 + m^2 + \dots + m^{2(H-1)} \leq m^{2H}$. In particular, the size of the extensive-form game $\calG'$ is polynomial as long as $H$ is bounded by a constant. In stark contrast, it is important to note that the normal-form representation of $\calG'$ is enormous---exponential even if $H = 2$; this why proving non-trivial hardness results for normal-form games (apparently) requires a different approach. Before we proceed with the main proof, we first have to recall some basic results regarding online density estimation.

\paragraph{Online density estimation.} Following~\citet{foster2023hardness}, our proof will invoke \emph{Vovk’s aggregating algorithm} for online density estimation~\citep{Vovk90:Aggregating}. In particular, the setting is as follows. (For consistency, we follow to a large extent the notation of~\cite{foster2023hardness} in the description below.) There are two players, the \emph{Nature} and the \emph{Learner}. There is a set $\calO$ called the \emph{outcome space}, and a set $\calC$ called the \emph{context space}; both may be assumed to be finite for our applications. The interaction between the Learner and the Nature proceeds for $t = 1, 2, \dots, T$ as follows.

\begin{enumerate}
    \item Nature first reveals a context $c^{(t)} \in \calC$;
    \item the Learner predicts a distribution $\hatvq^{(t)} \in \Delta(\calO)$ over outcomes based on the observed context $c^{(t)}$; and
    \item Nature chooses an outcome $o^{(t)} \in \calO$, and the Learner incurs a logarithmic loss defined as $\elllog^{(t)}(\hatvq^{(t)}) \defeq \log \left( \frac{1}{\hatvq^{(t)}(o^{(t)})} \right)$.
\end{enumerate}

We measure the regret against a (finite) set of experts $\calI$ . Every expert $i \in \calI$ corresponds to a function $p_i : \calC \to \Delta(\calO)$. The \emph{regret} of an algorithm with respect to the expert class $\calI$ is defined as
\begin{equation*}
    \reg_\calI^T \defeq \sum_{t=1}^T \elllog^{(t)}(\hatvq^{(t)}) - \min_{i \in \calI} \left\{ \sum_{t=1}^T \elllog^{(t)}(\vec{p}_i(c^{(t)}))  \right\}.
\end{equation*}

It is important to note here that the algorithm of the learner is allowed to observe the expert predictions $\{ \vec{p}_i(c^{(t)}) \}_{i \in \calI}$. In this context, Vovk's aggregating algorithm makes predictions via
\begin{equation}
    \label{eq:Vovk}
    \hatvq^{(t)} \defeq \E_{i \sim \tilvq^{(t)}}[\vec{p}_i(c^{(t)})], \textrm{ where } \tilvq^{(t)}(i) \defeq \frac{ \exp \left( - \sum_{\tau=1}^{t-1} \elllog^{(\tau)}(\vec{p}_i(c^{(\tau)})) \right) }{ \sum_{i' \in \calI} \exp \left( - \sum_{\tau=1}^{t-1} \elllog^{(\tau)}(\vec{p}_{i'}(c^{(\tau)})) \right) } \quad \forall i \in \calI.
\end{equation}

\begin{proposition}[\cite{Vovk90:Aggregating}]
    \label{prop:aggregation}
    If the distribution of outcomes is realizable under some $i^\star \in \calI$, then the predictions of the aggregation algorithm~\eqref{eq:Vovk} satisfy 
    \begin{equation*}
        \frac{1}{T} \sum_{t=1}^T \E \left[\dtv(\hatvq^{(t)}, \vec{p}_{i^\star}(c^{(t)})) \right] \leq \sqrt{ \frac{\log |\calI|}{T}}.
    \end{equation*}
\end{proposition}

We are now ready to proceed with the key proof of this section.

\begin{theorem}
    \label{theorem:inference-EFGs}
    Consider a $T$-sparse $\eps$-CCE (\Cref{def:sparseCCE}) in $\calG'$. \Cref{algo:EFG}, with $H \geq \frac{4 \log T}{\epsilon^2}$, computes a $2\epsilon$-Nash equilibrium in the two-player $m$-action game $\calG$ and runs in time $T \cdot \poly(m^H)$.
\end{theorem}

\begin{proof}
    We consider a sequence of product distributions $(\vec{X}_{1}^{(1)} \otimes \vec{X}^{(1)}_{2} , \dots, \vec{X}_1^{(T)} \otimes \vec{X}_{2}^{(T)})$ in $\calG'$ with the property that $\vec{\mu} \defeq \frac{1}{T} \sum_{t=1}^T \vec{X}_1^{(t)} \otimes \vec{X}_2^{(t)}$ is an $\epsilon$-CCE, and by construction $T$-sparse per \Cref{def:sparseCCE}. The goal is to show that there exists $t \in [T]$ and some state $s \in \calS$ such that $(\vec{x}_1, \vec{x}_2) \defeq (\vec{X}^{(t)}_{1, s}, \vec{X}^{(t)}_{2, s})$ is a $(2 \epsilon)$-Nash equilibrium; we recall that we use the notation $\vec{X}_{i, s} \in \Delta(\calA_i)$ to represent the strategy profile induced by $\vec{X}_i$ at state $s \in \calS$. We will show the claim by contradiction. 

    Indeed, for the sake of contradiction, suppose that for any $t \in [T]$ and $s \in \calS$, there is a player $i \in [2]$ who can come up with a deviation $\devX_{i, s}^{(t)}$ such that $u_i(\devX^{(t)}_{i, s}, \Vec{X}_{-i, s}^{(t)}) > u_i(\Vec{X}_s^{(t)}) + 2 \epsilon $, where $\vec{X}^{(t)}_s \defeq (\vec{X}^{(t)}_{1, s}, \vec{X}^{(t)}_{2, s})$. We will show that this contradicts the assumption that the correlated distribution $\Vec{\mu}$ is an $\epsilon$-CCE for $\calG'$.
    
    To do this, we suppose that each player $i$ uses the aggregation algorithm~\eqref{eq:Vovk} in order to estimate the strategy profile of the other player at every state. In particular, to relate our problem with the setup of online density estimation introduced earlier, we  make the following correspondence: 

    \begin{itemize}
        \item the context space $\calO$ corresponds to the set of all possible states $\calS$;
        \item the set of experts $\calI$ coincides with the set of indexes $[T]$; while
        \item the time index $t \in [T]$ in the context of online density estimation will now correspond to the repetition $h \in [H]$.
    \end{itemize}
       (There is an overload of notation here between the different settings, but we hope that this does not create any confusion.) Crucially, according to \Cref{def:sparseCCE}, player $i$ knows in advance the sequence of product distributions $(\vec{X}_{1}^{(1)} \otimes \vec{X}^{(1)}_{2} , \dots, \vec{X}_1^{(T)} \otimes \vec{X}_{2}^{(T)})$, which corresponds exactly to the set of experts in the context of online density estimation. On the other hand, and crucially, player $i$ does not know the index $t^\star$, which is sampled uniformly at random from $[T]$ and indicates which product distribution the other player is following. The basic idea is that, based on the opponent's actions throughout the game, each player can estimate the opponent's strategy as the game progresses. In this context, we can apply the aggregation algorithm~\eqref{eq:Vovk}, with context space corresponding to the history of the other player's actions, to obtain an estimate $\hatvq_{i, h} \in \Delta(\calA_{-i})$ for all repetitions $h \in [H]$. Now the deviation $\devX_i$ for player $i$ is defined so that in every possible state $s \in \calS$, it holds that $\devX_{i, s}$ is a best response to $\hatvq_{i, h(s)}$, where $h(s)$ represents the repetition corresponding to state $s \in \calS$.

    We next argue about the deviation benefit of player $i$ under $\devX_{i}$. In particular, we are interested in the payoff of player $i$ under the random process wherein we first draw an index $t^\star$ uniformly at random from the set $[T]$, player $i$ plays according to $\devX_i$, while the rest of the players play according to $\vec{X}^{(t^\star)}_{-i}$. By definition of this random process, realizability is satisfied: the observed distribution of outcomes obeys the law induced by $\vec{X}^{(t^\star)}_{-i}$, conditioned on the time index $t^\star$. As a result, \Cref{prop:aggregation} implies that for each player $i$ it holds that
    \begin{equation*}
        \E_{s_1, \dots, s_h} \left[ \sum_{h = 1}^H \dtv \left( \hatvq_{i, h}, \vec{X}^{(t^\star)}_{-i, s_h} \right) \right] \leq \sqrt{H \log T},
    \end{equation*}
    where the sequence of states $(s_1, \dots, s_h) \in \calS^H$ is drawn according to the random process described above. As a result, we conclude that for each player $i \in [2]$, conditioned on drawing $t^\star$ and being at repetition $h \in [H]$ and state $s_h \in \calS$,
    \begin{equation*}
        u_i(\devX_{i, s_h}, \vec{X}_{-i, s_h}^{(t^\star)}) \geq u_i(\devX_{i, s_h}, \hatvq_{i, h}) - \delta_{i, h}^{(t^\star)} \geq \max_{a_i \in \calA_i} \E_{a_{-i} \sim \vec{X}^{(t^\star)}_{-i, s_h} } u_i(a_i, a_{-i})  - 2 \delta_{i, h}^{(t^\star)},
    \end{equation*}
    where above we denoted by $\delta_{i, h}^{(t^\star)} \defeq \dtv \left( \hatvq_{i, h}, \vec{X}^{(t^\star)}_{-i, s_h} \right)$. Thus, 
    \begin{equation*}
        \sum_{i=1}^2 \left[ u_i(\devX_{i, s_h}, \vec{X}_{-i, s_h}^{(t^\star)}) - u_i(\vec{X}_{s_h}^{(t^\star)}) \right] > 2 \epsilon - 2 \delta_{i, h}^{(t^\star)},
    \end{equation*}
    which follows since we have assumed that the Nash equilibrium gap for all states $s \in \calS$ and $t \in [T]$ under $\vec{X}^{(t)}_{s}$ is strictly larger than $2 \epsilon$. Finally, taking the average of the draw $t^\star \in [T]$, which is chosen uniformly at random,
    \begin{align*}
        \frac{1}{T} \sum_{t=1}^T \sum_{i=1}^2 \left[ u'_i(\devX_i, \vec{X}^{(t)}_{-i}) - u_i'(\vec{X}^{(t)}) \right] &= \frac{1}{T H} \sum_{t=1}^T \sum_{i=1}^2 \sum_{h=1}^H \E_{s_1, \dots, s_h} \left[ u_i(\devX_{i, s_h}, \vec{X}^{(t)}_{-i, s_h}) - u_i(\vec{X}^{(t)}_{s_h}) \right] \\
        &> \frac{1}{H} \left( 2 \epsilon H - 2 \sqrt{H \log T} \right) \geq 2\epsilon - 2 \sqrt{\frac{\log T}{H}}.
    \end{align*}
    \io{The random process over $s_1, \dots, s_h$ is different depending on the deviation $\devX_i$, so the expression above is not correct.}
    As a result, for $H \geq 4 \frac{\log T}{\epsilon^2}$ it follows that $\vec{\mu}$ is not an $\epsilon$-CCE, which is a contradiction. This implies that \Cref{line:return} of \Cref{algo:EFG} will always be executed. Finally, the claimed running time of \Cref{algo:EFG} follows directly from the fact that the number of nodes of the extensive-form game $\calG'$ is bounded by $m^{2H}$.
\end{proof}

Below, for an extensive-form game $\calG'$, we denote by $|\calT'(\calG')|$ the number of nodes in the game-tree induced by $\calG'$.

\begin{corollary}
    Let $\calG'$ be any two-player extensive-form game. There is no algorithm that can compute a $\poly(\log |\calT'(\calG')|)$-sparse $\epsilon$-CCE in $\calG'$ in polynomial time even for an absolute constant $\epsilon > 0$, unless the exponential-time hypothesis for $\PPAD$ fails.
\end{corollary}

==> text/poa.tex <==
\section{Computing Equilibria that Match the Price of Anarchy}

\subsection{From Multi-Player Polymatrix to Two-Player Games}

Let $G = (\calN, E)$ be a directed graph associated with a polymatrix game. Each node $u \in \calN$ corresponds to a different player, and each edge $(u,v) \in E$ to a game between $u$ and $v$. Formally, each player $u \in \calN$ has a discrete action set $\calA_u$. Under strategies $(\vec{x}_{u})_{u \in \calN}$, the utility of each player $u \in \calN$ is given by
\begin{equation*}
    \sum_{v : (u,v) \in E} \vec{x}_u^\top \mat{A}_{u, v} \vec{x}_v,
\end{equation*}
where $\mat{A}_{u, v}$ represents the payoff matrix of the game that corresponds to the edge $(u, v)$. It is well-known that computing an approximate Nash equilibrium is $\PPAD$-hard in polymatrix games~\cite{Daskalakis09:The}. It also known that computing a welfare-maximizing \emph{correlated equilibrium (CE)} in polymatrix games is $\NP$-hard~\cite{Papadimitriou08:Computing}. (We still haven't found a proof of that in the literature.). We need the following stronger statement.

\begin{hypothesis}
Computing a welfare-maximizing CE remains $\NP$-hard even if the underlying graph $G$ is restricted to be $2$-colorable. (constant-colorable would probably suffice for our purposes.)
\end{hypothesis}

Restricting attention to $2$-colorable graphs is convenient since there is a natural reduction---in terms of computing (approximate) Nash equilibria---to two-player games. In two-player games, in turn, one can efficiently optimize over the set of correlated equilibria (assuming that the dimensions of the induced game are polynomial in the original description). The key difficulty is to understand whether there is an analogous reduction that also applies to correlated equilibria.

\paragraph{The reduction} The reduction from $2$-colorable polymatrix games to two-player games is based on~\cite{Daskalakis09:The}, although with a slight variation to lead to a two-player instead of a three-player instance. We assume that the nodes are partitioned into $\calN_1$ and $\calN_2$ which induce a valid coloring of the graph $G$. The idea is to use a meta-player, a ``lawyer,'' to represent each partition. Lawyer $1$ has action set the union $\bigcup_{u \in \calN_1} \calA_u$, while Lawyer $2$ has action set the union $\bigcup_{u \in \calN_2} \calA_u$. (It is crucial to consider the union instead of the product to maintain polynomial dimensions.) This naturally induces a two-player game $\Gamma$ between the laywers: Under actions $(u, a_u)$ and $(v, a_v)$, the utility of Lawyer $1$ is $0$ if $(u,v) \notin E$ and $\mat{A}_{u, v}[a_u, a_v]$ otherwise; the utility of Laywer $2$ is defined analogously. 

The hope now is that a Nash equilibrium pair $(\vec{X}_1, \vec{X}_2)$ in the induced game $\Gamma$ maps to an approximate Nash equilibrium in the original polymatrix game by taking the marginals for each node. This is not necessarily the case as laywers may be inclined in equilibrium to only represent a subset of their players; so, marginals in the above sense are not even well-defined. The simple way to address this consists of incorporating another ``high-stakes'' game between the laywers that enforces (approxiamtely) equal representation in equilibrium. In particular, let $M \gg 0$ be a large parameter, and assume for simplicity that $|\calN_1| = |\calN_2|$. We consider an arbitrary bijection between the sets $\calN_1$ and $\calN_2$. Then, the high-stakes games is a zero-sum game such that the utility of Laywer $1$ is $+M$ if the nodes selected by the laywers are in correspondence according to the bijection, and $0$ otherwise. Thus, we consider a game $\Gamma'$ in which the utility of each laywer is the sum of the utilities of the two games described above.

\begin{proposition}
    \label{prop:reduction-Nash}
Let $(\vec{X}_1, \vec{X}_2)$ be a Nash equilibrium in $\Gamma'$. If $\vec{x}_u[a_u] = \vec{X}_1[(u, a_u)]/\sum_{a_u' \in \calA_u} \vec{X}_1[(u, a_u')]$ for all $a_u \in \calA_u$ and $u \in \calN_1$, and similarly for nodes in $\calN_2$, then $(\vec{x}_u)_{u \in \calN}$ is an $O(1/M)$-approximate Nash equilibrium in the original game.
\end{proposition}

As a result, one can take $M$ to be arbitrarily large to complete the reduction. Our goal is to somehow extend~\Cref{prop:reduction-Nash} to the more general set of correlated equilibrium. 

In particular, let $\vec{\mu}$ be a correlated equilibrium in $\Gamma'$. The key question is whether $\vec{\mu}$ induces a correlated equilibrium in the original game. Perhaps the most natural choice is to consider the distribution over $\Delta(\prod \calA_u)$ such that 
\begin{equation*}
\Pr[(a_u)_{u \in \calN}] \propto \sum_{u \in \calN_1, v \in \calN_2} \vec{\mu}[(u, a_u), (v, a_v)].    
\end{equation*}
If $\vec{\mu}$ is a correlated equilibrium in $\Gamma'$, is the above distribution an $O(1/M)$-approximate correlated equilibrium in the original game?


==> text/randomized.tex <==
\section{Randomized Reduction}

Based on the extensive-form game $\calT$ described in \Cref{def:lifted-EFG}, our main reduction is summarized in \Cref{algo:EFG}. We clarify that the function $\textsc{NextState}(\cdot, \cdot)$ in \Cref{line:state} takes as input a state $s_h \in \calS$ along with a joint action $\va_h \in \bigtimes_{i=1}^3 \calA_i$, and returns the (unique) induced state $s_{h+1} \in \calS$; for $h = 0$, it is assumed by convention that the function returns $s_1$, that is, the root of the tree $\calT$.

It is evident that all steps in \Cref{algo:EFG} can be implemented in time polynomial in the description of $\calT$, with the exception of \Cref{line:CCE}, which depends on the underlying algorithm used to compute a sparse CCE. Along with \Cref{claim:nnodes}, we arrive at the following conclusion.

\begin{proposition}
    \label{prop:runtime}
    Let $\mathfrak{A}$ be an algorithm that takes as input an extensive-form game $\calT$ and computes a $T$-sparse $\epsilon$-CCE of $\calT$ in time at most $Q(|\calT|, T, 1/\epsilon)$. Then, \Cref{algo:EFG} instantiated with $\mathfrak{A}$ in \Cref{line:CCE} runs in time at most $Q(|\calT|, T, 1/\epsilon) +  T  m^{\Theta(H)}$.
\end{proposition}

\begin{remark}[Bit complexity of exponential weights]
    \Cref{line:EW} of \Cref{algo:EFG} updates $\tilvq_{i, h}^{(t)}$ using exponential weights (in accordance with the aggregation algorithm~\eqref{eq:Vovk}), which could result in $\tilvq_{i, h}^{(t)}$ taking irrational values. This can be addressed by truncating those values to the most significant $\log(|\calT|, T, H, 1/\epsilon)$ bits, in which case the proof of \Cref{theorem:inference-EFGs} readily carries over. For simplicity, we assume in our analysis that $\tilvq_{i, h}^{(t)}$ is updated per \Cref{line:EW}, without taking into account the numerical imprecision.
\end{remark}

It is worth commenting here on a couple of differences with the corresponding algorithm of~\citet{foster2023hardness}. First, \citet{foster2023hardness} had to encode the joint action profile through the reward, so as to ensure that each player has observed the prior sequence of joint actions. This is not necessary in our setting as, by construction, the states of the extensive-form game $\calT$  encode that information. \citet{foster2023hardness} also had to use a random sample to determine an approximate best response for the Kibitzer; in contrast, in our three-player setting \Cref{line:br} can be trivially implemented in $\poly(m)$ time.

\begin{algorithm}[!ht]
    \caption{Reduction for \Cref{theorem:inference-EFGs}}
    \label{algo:EFG}
    \textbf{Input}: Two-player $m$-action game $\calG$ in normal form; accuracy $\epsilon > 0$; sparsity $T \in \N$ \\
    \textbf{Output}: A $(18 \epsilon)$-Nash equilibrium of $\calG$ with probability at least $\frac{1}{2}$ \\
    Construct the three-player extensive-form game $\calT(\calG)$ with $H \geq \frac{\log T}{\epsilon^2}$ (\Cref{def:lifted-EFG}) \\
    Compute a $T$-sparse $\epsilon$-CCE $\frac{1}{T} \sum_{t=1}^T \bigotimes_{i=1}^3 \vx_i^{(t)}$ (\Cref{def:sparseCCE}) in $\calT$ \label{line:CCE} \\
    Draw $t^\star$ uniformly at random from the set $\range{T}$ \\
    \For{$h \in \range{H}$}{
    $s_h \defeq \textsc{NextState}(s_{h-1}, \va_{h-1}) \in \calS $ \label{line:state} \\
    For each player $i \in \range{2}$, let $\hatvq_{i, h} \defeq \E_{t \sim \tilvq_{i, h}} [ \vx^{(t)}_{i, s_h}] \in \Delta(\calA_i)$, where \\
    $$ \tilvq_{i, h}^{(t)} \defeq \frac{ \exp \left( - \sum_{\upsilon=1}^{h-1} \log \left( \frac{1}{\vx_{i, s_\upsilon}^{(t)}[a_{i, \upsilon}]} \right) \right) }{ \sum_{t' = 1}^T \exp \left( - \sum_{\upsilon=1}^{h-1} \log  \left(\frac{1}{ \vx_{i, s_{\upsilon}}^{(t')}[a_{i, \upsilon}] } \right) \right) } \quad \forall t \in \range{T} $$ \label{line:EW}\\
    Sample an action $\calA_i \ni a_{i, h} \sim \vx^{(t^\star)}_{i, s_h}$ for each player $i \in \range{2}$ \\
    Set $a_{\kib, h} \defeq \argmax_{ a'_{\kib, h} \in \calA_{\kib} } \E_{ a'_{1, h}, a'_{2, h} \sim \hatvq_{1, h}, \hatvq_{2, h} } u_{\kib, h}(\va'_{h})$ \label{line:br} \\
    \If{$(\hatvq_{1, h}, \hatvq_{2, h}) \in \Delta(\calA_1) \times \Delta(\calA_2)$ is an $(18 \epsilon)$-Nash equilibrium of $\calG$}{\textbf{return} $(\hatvq_{1, h}, \hatvq_{2, h}) \in \Delta(\calA_1) \times \Delta(\calA_2)$} \label{line:return}
    }
    \textbf{return} \textsf{FAIL}
\end{algorithm}

\subsection{From sparse CCE in $\calT$ to Nash equilibria in $\calG$}
\label{sec:inference}

We are now ready to proceed with the key proof of this section, which establishes the correctness of \Cref{algo:EFG}.

\begin{theorem}
    \label{theorem:inference-EFGs}
    When $H \geq \frac{ \log T}{\epsilon^2}$, \Cref{algo:EFG} returns an $(18 \epsilon)$-Nash equilibrium in the two-player $m$-action game $\calG$ with probability at least $\frac{1}{2}$.
\end{theorem}

\begin{proof}
    We consider a sequence of joint strategies $(\vx^{(1)}_1, \vx^{(1)}_2, \vx^{(1)}_3), \dots, (\vx^{(T)}_1, \vx^{(T)}_2, \vx^{(T)}_3) \in \bigtimes_{i=1}^3 \calX_i$ in the extensive-form game $\calT$ with the property that $\barvmu \defeq \frac{1}{T} \sum_{t=1}^T \bigotimes_{i=1}^3 \vx_i^{(t)}$ is an $\epsilon$-CCE, and by construction $T$-sparse per \Cref{def:sparseCCE}.
    
    Let us fix a player $i \in \range{3}$. We will first make use of the aggregation algorithm~\eqref{eq:Vovk}. In particular, for a player $i' \neq i$,  to relate our problem with the setup of online density estimation introduced earlier, we  make the following correspondence:
    \begin{itemize}
        \item the context space $\calO$ corresponds to the set of all possible decision nodes (or states) $\calS$ of the extensive-form game $\calT$;
        \item the set of experts $\calE$ coincides with the set $ \{ \vx_{i', s}^{(1)}, \dots, \vx_{i', s}^{(T)} \} $, with outcome space $\calA_{i'}$; while
        \item the time index $h \in \range{H}$ in the context of online density estimation will now fittingly correspond to the repetition $h \in \range{H}$.
    \end{itemize}
    Notice that, according to \Cref{def:sparseCCE}, player $i$ knows in advance the sequence of joint strategies $(\vx^{(1)}_1, \vx^{(1)}_2, \vx^{(1)}_3), \dots, (\vx^{(T)}_1, \vx^{(T)}_2, \vx^{(T)}_3) \in \bigtimes_{i=1}^3 \calX_i$. By construction of the extensive-form game $\calT$, player $i$ also observes the underlying state $s_h$ at each repetition $h \in \range{H}$. In this context, we will apply the aggregation algorithm~\eqref{eq:Vovk}, with the aforementioned parameterization, to obtain an estimate $\hatvq_{i', h} \in \Delta(\calA_{i'})$ for all repetitions $h \in \range{H}$ and $i' \neq i$. Namely,
    \begin{equation*}
        \hatvq_{i', h} \defeq \E_{t \sim \tilvq_{i', h}}[\vec{x}_{i', s_h}^{(t)}], \textrm{ where } \tilvq_{i', h}^{(t)} \defeq \frac{ \exp \left( - \sum_{\upsilon=1}^{h-1} \elllog_{\upsilon}(\vx_{i', s_\upsilon}^{(t)}) \right) }{ \sum_{t' = 1}^T \exp \left( - \sum_{\upsilon=1}^{h-1} \elllog_{\upsilon}(\vx_{i', s_\upsilon}^{(t')}) \right) } \quad \forall t \in \range{T}.
    \end{equation*}
    Above, we note that $\elllog_\upsilon( \vx^{(t)}_{i', s_\upsilon}) = \log \frac{1}{ \vx^{(t)}_{i', s_\upsilon}[a_{i', \upsilon}] }$. Now the deviation $\devX_{i, h} \in \Delta(\calA_i) $ for player $i \in \range{3}$ is defined as follows.
       \begin{equation}
            \label{eq:devq}
           \devX_{i, h} \defeq \argmax_{a_{i, h} \in \calA_i} \E_{\vec{a}_{-i, h} \sim \bigtimes_{i' \neq i} \hatvq_{i', h}} [u_{i, h}(a_{i, h}, \va_{-i, h})].
       \end{equation}
    We next argue about the deviation benefit of player $i$ under the strategy $\devX_{i}$ induced by the random process described above. In particular, we are interested in the payoff player $i$ obtains under the random process wherein we first draw an index $t^\star$ uniformly at random from the set $\range{T}$, player $i$ plays according to the deviation strategy $\devX_i$, while the rest of the players play according to $\vx^{(t^\star)}_{-i}$. By definition of this random process, realizability is satisfied: the observed distribution of outcomes obeys the law induced by $\vx^{(t^\star)}_{i'} : \calS \to \Delta(\calA_{i'})$, conditioned on the time index $t^\star$. As a result, \Cref{prop:aggregation} implies that for each player $i \in \range{3}$ and $i' \neq i$ it holds that
    \begin{equation}
        \label{eq:TV-close}
        \E_{ \devX_i \times \vx_{-i}^{(t^\star)}} \left[ \sum_{h = 1}^H \dtv \left( \hatvq_{i', h}, \vx^{(t^\star)}_{i', s_h} \right) \right] \leq \sqrt{H \log T},
    \end{equation}
    where the expectation and the sequence of states $(s_1, \dots, s_H) \in \calS^H$ is taken with respect to the random process described above.

    Furthermore, we have that
    \begin{align}
        u_i(\devX_i, \barvmu_{-i}) &= \E_{t^\star \sim \uni(\range{T})} [ u_i(\devX_i, \vx_{-i}^{(t^\star)}) ] = \E_{t^\star \sim \uni(\range{T})} \E_{ \devX_i, \vx_{-i}^{(t^\star)}} \sum_{h=1}^H \E_{\va_{-i, h} \sim \vx^{(t^\star)}_{-i, s_h}} [u_{i, h}( \devX_{i, h}, \va_{-i, h} )] \notag \\
        &\geq - 2 \sqrt{\frac{\log T}{H}} + \E_{t^\star \sim \uni(\range{T})} \E_{ \devX_i, \vx_{-i}^{(t^\star)}} \sum_{h=1}^H \E_{\va_{-i, h} \sim \hatvq_{-i, h}  } [u_{i, h}( \devX_{i, h}, \va_{-i, h} )] \label{align:TV-sum} \\
        &\geq - 2 \sqrt{\frac{\log T}{H}} + \E_{t^\star \sim \uni(\range{T}) } \E_{ \devX_i, \vx_{-i}^{(t^\star)}} \sum_{h=1}^H \max_{a_{i, h} \in \calA_i} \E_{\va_{-i, h} \sim \hatvq_{-i, h}} [u_{i, h}( a_{i, h}, \va_{-i, h} )] \label{align:opt-dev} \\
        &\geq- 2 \sqrt{\frac{\log T}{H}},\label{align:product-nonnegative}
    \end{align}
    where \eqref{align:TV-sum} uses~\eqref{eq:TV-close} along with the fact that 
    \begin{align*}
        \E_{\va_{-i, h} \sim \vx^{(t^\star)}_{-i, s_h}} [u_{i, h}( \devX_{i, h}, \va_{-i, h} )] &\geq \E_{\va_{-i, h} \sim \hatvq_{-i, h}  } [u_{i, h}( \devX_{i, h}, \va_{-i, h} )] - \frac{1}{H} \dtv\left( \vx^{(t^\star)}_{-i, s_h}, \bigtimes_{i' \neq i} \hatvq_{i', h}  \right) \\
         &\geq \E_{\va_{-i, h} \sim \hatvq_{-i, h}  } [u_{i, h}( \devX_{i, h}, \va_{-i, h} )] - \frac{1}{H} \sum_{i' \neq i} \dtv\left( \vx^{(t^\star)}_{i', s_h},  \hatvq_{i', h}  \right), 
    \end{align*}
    since $|u_{i,h}(\cdot, \cdot)| \leq \frac{1}{H}$ (by construction), and the total variation distance between two product distributions is bounded by the sum of the total variation of the individual components~\citep{Hoeffding58:Distinguishability}; \eqref{align:opt-dev} follows from the definition of $\devX_{i, h}$ in~\eqref{eq:devq}, which in particular implies that 
    $$\E_{\va_{-i, h} \sim \hatvq_{-i, h}  } [u_{i, h}( \devX_{i, h}, \va_{-i, h} )] = \max_{a_{i, h} \in \calA_i} \E_{\va_{-i, h} \sim \hatvq_{-i, h}} [u_{i, h}( a_{i, h}, \va_{-i, h} )];$$ and~\eqref{align:product-nonnegative} follows from the fact that $\max_{a_{i, h} \in \calA_i} \E_{\va_{-i, h} \sim \hatvq_{-i, h}} [u_{i, h}( a_{i, h}, \va_{-i, h} )] \geq 0$ (\Cref{lemma:nonnegativity}). Further, given that $\barvmu$ is assumed to be an $\epsilon$-CCE, \eqref{align:product-nonnegative} implies that for each player $i \in \range{3}$,
    \begin{equation}
        \label{eq:aux}
        u_i(\barvmu) \geq - 2 \sqrt{\frac{\log T}{H}} - \epsilon. 
    \end{equation}
    
    Given that $\calT$ is zero-sum, we also have that $\sum_{i=1}^3 u_i(\barvmu) = 0$; by~\eqref{eq:aux}, this in turn implies that $u_\kib(\barvmu) = - u_1(\barvmu) - u_2(\barvmu) \leq 4 \sqrt{\frac{\log T}{H}} + 2 \epsilon$.
    
    We next focus on analyzing the deviation benefit of the Kibitzer. By~\eqref{align:opt-dev}, we have that the utility $u_\kib(\devX_\kib, \barvmu_{-\kib})$ can be lower bounded by
    \begin{align*}
         \frac{1}{H} \E_{t^\star \sim \uni(\range{T})} \E_{ \devX_\kib, \vx_{-\kib}^{(t^\star)}} \sum_{h=1}^H \max_{i' \in \range{2}, a'_{i', h} \in \calA_{i'}} \E_{\va_{-\kib, h} \sim \hatvq_{-\kib, h}} [\mat{M}_{i'}[a_{i', h}', \va_{-i', h}] - \mat{M}_{i'}[\va_h]] - 2 \sqrt{\frac{\log T}{H}}.
    \end{align*}
    
    Now, since $\barvmu$ is an $\epsilon$-CCE, we also have that $u_\kib(\devX_\kib, \barvmu_{-\kib}) \leq u_\kib(\barvmu) + \epsilon \leq 3 \epsilon + 4 \sqrt{\frac{\log T}{H}}$. Finally, given that $\max_{i' \in \range{2}, a'_{i', h} \in \calA_{i'}} \E_{\va_{-i, h} \sim \bigtimes_{i' \neq i} \hatvq_{i', h}} [\mat{M}_{i'}[a_{i', h}', \va_{-i', h}] - \mat{M}_{i'}[\va_h] ] \geq 0$ (\Cref{lemma:nonnegativity}), Markov's inequality implies that with probability at least $\frac{1}{2}$ over $t^\star \sim \uni( \range{T})$ and the trajectory induced by the joint strategy $\devX_\kib, \vx_{-\kib}^{(t^\star)}$, there is some $h \in \range{H}$ such that
    \begin{equation*}
        \max_{i' \in \range{2}, a'_{i'} \in \calA_{i'}} \E_{\va_{-i, h} \sim \bigtimes_{i' \neq i} \hatvq_{i', h}} [\mat{M}_{i'}[a_{i', h}', \va_{-i', h}] - \mat{M}_{i'}[\va_h] ] \leq 6 \epsilon + 12 \sqrt{\frac{\log T}{H}} \leq 18 \epsilon.
    \end{equation*}
\end{proof}

==> text/sparse-NFGs.tex <==
\section{Hardness of Sparse CCE in Normal-Form Games}
\label{sec:NFGs}



The starting point of our reduction is a \emph{graphical game} $\calG$, associated with a graph $G = (V, E)$. The key property of graphical games is that the utility of each player $i$, uniquely associated with a node in $V$, depends solely in the actions of the neighbors $\calN_i \defeq \{u \in V : (i,u) \in E\}$. It is further assumed that $|\calN_i| \leq \Delta$, for some constant $\Delta \geq 2$, so as to ensure a compact representation of the game. An important property we need regarding equilibrium computation in graphical games is the following hardness result~\cite{Rubinstein18:Inapproximability}.


\begin{theorem}[\cite{Rubinstein18:Inapproximability}]
    \label{theorem:ppad-graphical}
    Computing an $\epsilon$-Nash equilibrium in a binary-action graphical game with bounded degree is $\PPAD$-hard, even for an absolute constant $\epsilon > 0$.
\end{theorem}

Indeed, it turns out that Nash equilibria in binary-action bounded-degree graphical games can be used to implement generalized circuits, which is in turn $\PPAD$-hard even for a constant $\epsilon > 0$. As a result, for the rest of our reduction we can restrict attention to the case where $|\calA_i| = 2$, for all $i \in [n]$.


Now the main step in the reduction is to construct a new ``lifted'' game, similarly to~\cite{foster2023hardness}, so as to use \emph{sparse} CCE in the lifted game in order to compute (approximate) Nash equilibria in the original game.

\paragraph{The lifted game.} We will first describe the lifted game as an (imperfect-information) extensive-form game, which is more natural, but we will then work with the normal-form representation of the lifted game. Building on the approach of~\cite{foster2023hardness} in the context of finite-horizon Markov games, we consider an (imperfect-information) extensive-form game which is obtained from $\calG$ through $H$ repetitions, for a suitable chosen parameter $H \in \N$. In each repetition $h \in [H]$, every player $i \in [n]$ observes a state $s^{(h)}_i$; subsequently, all players select simultaneously an action $a^{(h)}_i \in \calA_i$. More precisely, the information structure of the game is such that the state $s_i$ fully encodes the history of actions played by the players in the neighborhood of $\calN_i$ before the $h$-th repetition; it is crucial that $s_i$ only encodes the actions of the neighboring players, for otherwise the induced normal-form representation would be too large to render our reduction of any algorithmic use. Moreover, the utility of player $i$ is given by $u_i'(a_1', \dots, a_n') \defeq \frac{1}{H} \sum_{h=1}^H u_i(a_{1, h}, \dots, a_{n, h})$, where $a_i' \defeq (a_{i, 1}, \dots, a_{i, H}) \in \calA_i^H$.

Now the number of possible states a player $i \in [n]$ can encounter is upper bounded by $1 + 2^\Delta + \dots + 2^{(H-1) \Delta} \leq 2^{H \Delta}$. Further, in each possible state the player has a binary decision. If we let $\calA_i'$ be the action set of player $i$ in the lifted game $\calG'$ represented in normal form, each action in $\calA_i'$ should fully specify $i$'s actions in every possible state that can be encountered in the game. Thus, the following bound is immediate.

\begin{claim}
It holds that $|\calA_i'| \leq 2^{2^{H \Delta}}$.
\end{claim}

For convenience, we will let $m' \triangleq \max_i |\calA_i'| \leq 2^{2^{H \Delta}}$. This bound is crucial in order to obtain meaningful hardness results for normal-form games. Furthermore, it is evident that we cannot afford to write the lifted game $\calG'$ explicitly since that would require specifying $\exp(n)$ quantities. Nevertheless, it suffices if $\calG'$ has the polynomial expectation property (with respect to the description of $\calG'$), which is evident since $\calG'$ remains a bounded-degree graphical game.

\begin{claim}
    For any player $i \in [n]$ and for any strategy profile $\vec{x}'_{-i}$ in $\calG'$, we can compute the expectation $\E_{\vec{a}'_{-i} \sim \vec{x}'_{-i}} [u_i'(a_i', \vec{a}_{-i}')]$ in time $\poly(n, m')$, for any $a_i' \in \calA_i'$.
\end{claim}

The key step in the proof is the following theorem, which guarantees that a sparse $\epsilon$-CCE in $\calG'$ can be used to compute an $\epsilon$-Nash in $\calG$.

\begin{theorem}
    \label{theorem:inference}
    Consider a $k$-sparse $\epsilon$-CCE in $\calG'$. For a sufficiently large $H = O(\log k/\epsilon^2)$, there is an algorithm that computes an $O(\epsilon)$-Nash equilibrium in $\calG$ and runs in time $\poly(n, m', k)$.
\end{theorem}

The proof is similar to~\cite{foster2023hardness}, and relies on \emph{online density estimation}. 



\begin{proof}[Proof of \Cref{theorem:inference}]
    We consider a sequence of product distributions $(\vec{X}^{(1)}, \dots, \vec{X}^{(T)})$ in $\calG'$, that is, $\vec{X}^{(t)} \in \bigotimes_{i=1}^n \calA_i$, with the property that $\frac{1}{T} \sum_{t=1}^T \vec{X}^{(t)}$ is an $\epsilon$-CCE (and by construction $T$-sparse per \Cref{def:sparseCCE}).

    The goal is to show that there exists $t \in [T]$ and some state $\calS \ni s \mapsto (s_1, \dots, s_n)$ such that $\vec{X}^{(t)}_s \defeq (\vec{X}^{(t)}_{1, s_1}, \dots, \vec{X}^{(t)}_{n, s_n}) $ is an $O(\epsilon)$-Nash equilibrium, under some absolute constant. We will show this by contradiction. 

    For the sake of contradiction, suppose that for any $t \in [T]$ and $s \in \calS$, there is a player $i \in [n]$ who can come up with a deviation $\devX_{i, s_i}^{(t)}$ such that $u'_i(\devX^{(t)}_{i, s_i}, \Vec{X}_{-i, s_{-i}}^{(t)}) \geq u'_i(\Vec{X}_s^{(t)}) + C \epsilon $, for a sufficiently large absolute constant $C > 0$ to be determined. We will show that this contradicts the assumption that the correlated distribution $\frac{1}{T} \sum_{t=1}^T \vec{X}^{(t)}$ is an $\epsilon$-CCE. To do this, player $i$ will use the aggregation algorithm~\eqref{eq:Vovk} in order to estimate the joint distribution of the other players $-i$. 
    
    In particular, to relate our problem with the setup of online density estimation introduced earlier, we note that the context space corresponds to the set of possible history of play as observed by player $i$, and the set of experts $\calI$ coincides with the set of indexes $[T]$. According to \Cref{def:sparseCCE}, player $i$ knows the sequence of products $(\vec{X}^{(1)}, \dots, \vec{X}^{(T)})$, but player $i$ does not know the index $t^\star$, which is sampled uniformly at random from $[T]$ and indicates which product the rest of the players are playing according to. As a result, applying the aggregation algorithm~\eqref{eq:Vovk} induces an estimate $\hatvq_{i, s_i}$ for all states $s_i \in \calS_i$. Now the deviation $\devX_i$ for player $i$ is defined so that in every possible state of player $i \in [n]$ $\devX_{i, s_i}$ is a best response to $\hatvq_{i, s_i}$.

    We next argue about the deviation benefit of player $i$ under $\devX_{i}$. We are interested in the payoff of player $i$ under the random process wherein we first draw an index $t^\star$ uniformly at random from the set $[T]$, player $i$ plays according to $\devX_i$, while the rest of the players play according to $\vec{X}^{(t^\star)}_{-i}$. By definition of this random process, realizability is satisfied: the observed distribution of outcomes obeys the law induced by $\vec{X}^{(t^\star)}_{-i}$, conditioned on the time index $t^\star$. As a result, \Cref{prop:aggregation} implies that player $i$ can accurately perform the estimation step, in the sense that
    \begin{equation*}
        \E_{} \left[ \sum_{h = 1}^H \dtv \left( \hatvq_{i, s_i}, \vec{X}^{(t^\star)}_{-i}(c^{(h)}) \right) \right] \leq \sqrt{H \log T}.
    \end{equation*}
    Thus, by taking $H = C' \log T/\epsilon^2$, for a sufficiently large constant $C'$, and using the fact that player $i$ always has an $O(\epsilon)$ profitable deviation, we conclude that $\devX_i$ yields an $O(\epsilon)$ profitable deviation, which contradicts the assumption that the joint distribution is an $\epsilon$-CCE.
\end{proof}

\begin{corollary}
There is no algorithm that, given a multi-player game $\calG'$ with the polynomial expectation property, computes an $O(1)$-sparse $\epsilon$-CCE in time $\poly(\calG')$, unless $\PPAD \subseteq \P$.
\end{corollary}

\begin{proof}
By \Cref{theorem:inference}, an algorithm for computing $O(1)$-sparse CCE in $\poly(\calG')$ would yield an $\FPTAS$ for computing an $\epsilon$-Nash equilibrium in binary-action constant-degree graphical games. The conclusion then follows from~\Cref{theorem:ppad-graphical}.
\end{proof}

A more careful argument implies the following stronger lower bound.

\begin{corollary}
    Let $\calG'$ be a multi-player game with the polynomial expectation property and $|\calA_i'| \leq m$, for some $m \in \N$. There is an absolute constant $\delta > 0$ such that no algorithm computes an $O(\log^\delta m)$-sparse $\epsilon$-CCE in time $\poly(\calG')$, unless $\PPAD \subseteq \P$, where $\epsilon$ is a sufficiently small absolute constant.
\end{corollary}
